Domain Adaptive Decision Trees: Implications for Accuracy and Fairness

In uses of pre-trained machine learning models, it is a known issue that the target population in which the model is being deployed may not have been reflected in the source population with which the model was trained. This can result in a biased model when deployed, leading to a reduction in model performance. One risk is that, as the population changes, certain demographic groups will be under-served or otherwise disadvantaged by the model, even as they become more represented in the target population. The field of domain adaptation proposes techniques for a situation where label data for the target population does not exist, but some information about the target distribution does exist. In this paper we contribute to the domain adaptation literature by introducing domain-adaptive decision trees (DADT). We focus on decision trees given their growing popularity due to their interpretability and performance relative to other more complex models. With DADT we aim to improve the accuracy of models trained in a source domain (or training data) that differs from the target domain (or test data). We propose an in-processing step that adjusts the information gain split criterion with outside information corresponding to the distribution of the target population. We demonstrate DADT on real data and find that it improves accuracy over a standard decision tree when testing in a shifted target population. We also study the change in fairness under demographic parity and equal opportunity. Results show an improvement in fairness with the use of DADT.

==> previous_version/NotesSR.tex <==
\newpage

\section{Introduction}
\label{sec:Introduction}
When implementing the use of pre-trained machine learning models, it is a known issue that the target population in which the model is being deployed may not have been reflected in the data with which the model was trained. There are many reasons why a training set would not match the the target population, including the following:
\begin{itemize}
    \item Selection bias, wherein due to some \textit{(self-)selection mechanism} the training data does not represent the population that it was drawn from.
    \item Change in target population over time.
    \item The training set was drawn from one population but the target population is different (ex. different geography).
\end{itemize}

One, often advisable, approach to deal with this is to train a new model with updated or improved training data. However, there are cases where renewed data collection is not possible (such as if the required information is not known), or not desirable (cost, financial and otherwise is often mentioned as a barrier). A specific case of the information not being known is when we do not have labeled instances in the target domain. The field of domain adaptation proposes techniques for this situation.

In this paper we contribute to the domain adaptation literature by introducing {\em domain-adaptive decision trees} (DADT). We focus on decision trees given their popularity, interpretability relative to other ML models. With DADT we are able to improve accuracy of models trained in a  source domain that differs from the target domain (as may occur when we do not have labeled instances for the target domain). We do this by proposing an in-processing step that augments the Information Gain (IG) split criterion with outside information (but not label data), corresponding to the target population we aim for. 

Our proposal is intended to address a specific kind of domain shift, that is \emph{covariate shift}, where only the distribution of the attributes change (not the relationship between the attributes and the label). A relevant scenario would be... Our proposal would be relevant in a situation where we have some knowledge about population changes...


The paper is organized as follows. We present a short related work section situating our approach in the literature on domain adaptation in decision trees and adjusting the information gain of decision trees, we then introduce the problem setting as a domain adaptation problem and specifically focus on the covariate shift type of this problem:. We present the necessary background information on decision trees and information gain, before presenting our proposed intervention to information gain in \ref{sec:DADT}. In \ref{sec:Experiments} we present the results of our experiments on real and synthetic data. We then examine those results to understand the impact of our intervention under different kind of distribution shift. We see that our intervention leads to an increase in accuracy when the covariate shift assumption holds.


\section{Related Work}
\label{sec:RelatedWork}

Folktables a dataset for studying the impact of domain shift and domain drift ``What does the sensitivity to distribution shift say about algorithmic tools developed in one context and deployed in another? Answers to these questions seem highly relevant to policy-making around the deployment of algorithmic risk assessment tools.'' \cite{dingRetiringAdultNew2021}. The experiments presented focus on understanding the impact of shifts on fariness metrics (and fairness interventions).

Recent work has examined the relationship between domain adaptation and and fairness metrics. \cite{mukherjeeDomainAdaptationMeets2022} show that under some circumstances individual fairness techniques can improve domain adaptation, and that domain adaptation techniques can enforce individual fairness (this seems to be due to some probablistic connection between DA and IF). A related work to check \cite{maityDoesEnforcingFairness}.

Domain adaptation is a category of transfer learning. Transfer learning is the term for a machine learning algorithms that are intended to work in a learning setting where the training and test data are not assumed to have been drawn from populations with the same probability distributions. Domain adaptation specifically refers to transfer learning cases where the source and the target tasks are the same, but where we have labeled instances only for the source dataset \cite{Redko2020_DASurvey}.

In this paper we propose an approach to domain adaptation for decision trees, based on an intervention in the information gain (IG) calculation. To the best of our knowledge, we are the first to do a domain adaptation interpretation of the IG, and to modify the inherent weight provided by definition of $IG$ rather than incorporating a new weight. \cite{guiasu_weighted_1971} proposes a weighted entropy where $P(x)$ remains unchanged. Similarly, \cite{DBLP:journals/eswa/SingerAB20} proposes a weighted IG for capturing the risk of a portfolio of financial products. They use the values of the financial products to weight conditional entropy term of the IG when constructing the DT. Also, from a fairness perspective, \cite{DBLP:conf/ijcai/ZhangN19} weight the conditional entropy by considering parity between the classes of a protected attribute such that information gains are adjusted for potential unfair decision outcomes by the DT. 



% TODO: move into sections/ProblemSetting.tex
\section{Problem Setting}
\label{sec:ProblemSetting}

We assume a scenario in which the population used for training a classifier (the \textit{source domain} $D_S$) is not representative of the population over which the classifier is applied to (the \textit{target domain} $D_T$). Both populations are defined by a set of $m$ \textit{predictive attributes} $\mathbf{X}$ and a \textit{class attribute} $Y$. The predictive attributes can be discrete or continuous, while the class attribute is discrete. 
A classifier is a function $f()$ of the predictive attributes. In particular, we focus on decision tree classifiers. We denote by $\hat{Y}$ the \textit{predicted class} of the \textit{classifier} $f$, such that $\hat{Y} = f(\mathbf{X})$. We use uppercase letters for random variables and lowercase letters for their assignments. Therefore, $\hat{y} = f(\mathbf{x})$ represents the predicted class value for the instance $\mathbf{X}=\mathbf{x}$ .

The joint probability distributions are denoted by $P_S(\mathbf{X}, Y)$ and $P_T(\mathbf{X}, Y)$ for the source and target domain, respectively. 
The assumed scenario is tackled as a domain adaptation problem \cite{Redko2020_DASurvey} where $P_S(\mathbf{X}, Y) \neq P_T(\mathbf{X}, Y)$. Changes between the distributions are referred to as \textit{distribution shifts}. There are three types of distributions shifts \cite{Quinonero2009,DBLP:journals/pr/Moreno-TorresRACH12}. 
\textit{Covariate shift}: only the distribution of the attributes changes, $P_S(Y | \mathbf{X}) = P_T(Y | \mathbf{X})$ but $P_S(\mathbf{X}) \neq P_T(\mathbf{X})$.
\textit{Prior probability shift}: only the distribution of the class changes, $P_S(\mathbf{X}|Y) = P_T(\mathbf{X}|Y)$ but $P_S(Y) \neq P_T(Y)$. 
And \textit{dataset shift}: when none of the two previous cases apply but the joint distributions differ, $P_S(\mathbf{X}, Y) \neq P_T(\mathbf{X}, Y)$.

We focus on the covariate shift type \cite{DBLP:conf/icml/ZhangSMW13}. 
In particular, we consider its \textit{unsupervised case} in which we only have access to information on the target domain with regard to the predictive attribute distribution $\hat{Y}$, not on the class distribution $Y$. 
The unsupervised covariate shift case covers situations in which we need to make a prediction on $D_T$ using information from $D_S$, but are aware that the available source information is not representative of the needed target information for the classifier, i.e., $P_S(\mathbf{X}) \neq P_T(\mathbf{X})$.
Therefore, what can be done to address this situation depends on how much is known about $P_T(\mathbf{X})$.

In the ideal limit case where we know the whole covariate distribution $P_T(\mathbf{X})$, the assumption of covariate shift allows for computing the full distribution because of the multiplication rule of probabilities:
%
\begin{equation}
\label{eq:chain}
   P_T(Y, \mathbf{X}) = P_T(Y | \mathbf{X}) \cdot P_T(\mathbf{X}) = P_S(Y | \mathbf{X}) \cdot P_T(\mathbf{X})
\end{equation}
%
where we can exchange $P_T(Y|\mathbf{X})$ for $P_S(Y|\mathbf{X})$, which is convenient as we know both $Y$ and $\mathbf{X}$ in $D_S$. In reality, however, the right-hand-side of \eqref{eq:chain} can only be known to some extent due to three potential issues:
\begin{enumerate}
    \item[(P1)] $P_T(\mathbf{X})$ is not fully available, e.g., only the marginal distributions of some of the attributes $X \in \mathbf{X}$ are known;
    \item[(P2)] $P_T(Y | \mathbf{X}) \approx P_S(Y | \mathbf{X})$ but they are not exactly the same, i.e.,  covariate shift holds in a relaxed form; and
    \item[(P3)] $P_T(\mathbf{X})$ and $P_S(Y | \mathbf{X})$ are estimated given a sample data from the respective populations, and, as such, the estimation can have some variability. 
\end{enumerate}
The issue P3 is pervasive in statistical inference and machine learning. We do not explicitly\footnote{We tackle it implicitly through the Law of Large Numbers by restricting to estimation of probabilities in contexts with a minimum number of instances. This is managed in decision tree learning by a parameter that stops splitting a node if the number of instances at a node is below a minimum threshold.} consider it in our problem statement. Therefore, the main research question that we intend to address in this paper is:

\smallskip
\textit{RQ\textcolor{red}{1}. With reference to the decision tree classifiers, which type and amount of target domain knowledge (issue P1) can help to reduce the loss in accuracy at the variation of relaxed covariate shift (issue P2)?}

\smallskip
\textcolor{red}{In the interest of fairness, as $P_T(\mathbf{X})$ might contain sensitive information used by the decision tree classifier we wish to train, a subsequent question to address in this paper is:}

\smallskip
\textcolor{red}{\textit{RQ2. How is the loss in accuracy by the decision tree classifier, based on the issues P1 and P2, affect a fairness metric used for protected groups of interest in the target domain?}}

\smallskip
The range of cases to consider for both RQ1 and RQ2 span two opposites. 
\textbf{\textit{No target domain knowledge.}} This case consists of training a decision tree on the source data and using it on the target data, without any change or correction. Formally, we estimate $P_T(\mathbf{X})$ as $P_S(\mathbf{X})$ and $P_T(Y | \mathbf{X})$ as $P_S(Y | \mathbf{X})$.
\textbf{\textit{Full target domain knowledge.}} This case consists of training a decision tree on the source data and using it on the target data, but exploiting full knowledge of $P_T(\mathbf{X})$ in the learning algorithm.
\textbf{\textit{Partial target domain knowledge}}. Consequently, the in-between case consists of training a decision tree on the source data and using it on the target data, but exploiting partial knowledge of $P_T(\mathbf{X})$ in the learning algorithm and complementing it with knowledge of $P_S(\mathbf{X})$.

% \smallskip
% The range of cases to consider for both RQ1 and RQ2 span from two opposites:
% \begin{description}
%     \item[\textit{No target domain knowledge.}] This consists of training a decision tree on the source data and using it on the target data, without any change or correction. Formally, we estimate $P_T(\mathbf{X})$ as $P_S(\mathbf{X})$ and $P_T(Y | \mathbf{X})$ as $P_S(Y | \mathbf{X})$. 
%     %
%     \item[\textit{Full target domain knowledge.}] This consists of training a decision tree on the source data and using it on the target data, but exploiting full knowledge of $P_T(\mathbf{X})$ in the learning algorithm. 
% \end{description}

We specify how to exploit the knowledge of $P_T(\mathbf{X})$ for a decision tree classifier in Section~\ref{sec:DADT}, introducing what we refer to as a \textit{domain-adaptive decision tree} classifier.
Before answering this question, we introduce the required technical background on decision tree learning in the remainder of this section. 
   
% From a technical side, we need to specify how to exploit the (full or partial) knowledge of $P_T(\mathbf{X})$ in the learning algorithm. Before answering this question, we introduce more technical background on decision tree induction. 

% \section{Background}

\subsection{Decision Tree Learning}
\label{sec:ProblemSetting.DecisionTreeLearning}

% Decision trees are intuitive, interpretable, and popular classification models. 
Top-down induction algorithms grow a decision tree classifier \cite{Hastie2009_ElementsSL} from the root to the leaves. At each node, either the growth stops producing a leaf, or a split condition determines child nodes that are recursively grown. 
%
Common stopping criteria include node purity (all instances have the same class value), data size (the number of instances is lower than a threshold), and tree depth (under a maximum depth allowed). Split conditions are evaluated based on a split criterion, which selects one of them or possibly none (in this case the node becomes a leaf). 
%
We assume binary splits\footnote{There are other forms of binary, multi-way and multi-attribute split conditions.} of the form: $X=t$ for the left child and $X\neq t$ for the right child, when $X$ is a discrete attribute; or $X\leq t$ for the left child and $X > t$ for the right child, when $X$ is a continuous attribute. 

We call $X$ the \textit{splitting attribute}, and $t \in X$ the \textit{threshold value}. Together they form the \textit{split condition}.
%
Instances of the training set are passed from a node to its children by partitioning them based on the split condition.
%
The conjunction of split conditions from the root to the current node being grown is called the \textit{current path} and it is denoted by $\varphi$.
% In other words, 
It determines the instances of the training dataset being considered at the current node. The predicted probability of class $y$ at a leaf node is an estimation of $P(Y=y|\varphi)$ obtained by the relative frequency of $y$ among the instances of the training set reaching the leaf or, equivalently, satisfying $\varphi$.

\subsection{Entropy and the Information Gain Split Criterion}
\label{sec:ProblemSetting.Entropy}

We focus on the Information Gain split criterion. It is, along with Gini, one of the standard split criteria used. It is also based on information theory via entropy \cite{Cover1999ElementsIT}, which links a random variable's distribution to its information content. The \textit{entropy} ($H$) measures the information contained within a random variable based on the uncertainty of its events. The standard definition used is \textit{Shannon's entropy} \cite{DBLP:conf/icaisc/MaszczykD08} where we define $H$ for the class random variable $Y$ at $\varphi$ as:
%
\begin{equation}
\label{eq:ShannonEntropy}
            H(Y|\varphi) = \sum_{y \in Y} - P(Y=y|\varphi) \log_2(P(Y=y|\varphi))
\end{equation}
%
where $-\log_2(P(Y=y|\varphi))=I(y|\varphi)$ represents the \textit{information} ($I$) of $Y=y$ at current path $\varphi$. Therefore, entropy is the expected information of the class distribution at the current path. 
%
Intuitively, the information of class value $y$ is inversely proportional to its probability $P(Y=y|\varphi)$. The more certain $y$ is, reflected by a higher $P(Y=y|\varphi)$, the lower its information as $I(y|\varphi)$ (along with its contribution to $H(Y|\varphi)$). The general idea behind this is that there is little new information to be learned from an event that is certain to occur. 
% We picture it as \textit{low entropy implies no surprises}. 

The \textit{information gain} ($IG$) for a split condition is the difference between the entropy at a node and the weighted entropy at the child nodes determined by the split condition in consideration. For a discrete splitting attribute $X$ and threshold $t$, we have:
%
\begin{align}
\label{eq:BasicIGd}
    IG(X, t | \varphi) =  H(Y|\varphi) - P(X=t|\varphi) H(Y|\varphi, X=t) - P(X\neq t|\varphi) H(Y|\varphi, X \neq t)
\end{align}
%
and for a continuous splitting attribute $X$ and threshold $t$:
%
\begin{align}
\label{eq:BasicIGc}
    IG(X, t | \varphi) =  H(Y|\varphi) - P(X\leq t|\varphi) H(Y|\varphi, X\leq t) - P(X> t|\varphi) H(Y|\varphi, X > t)
\end{align}
%
The selected split attribute and threshold are those with maximum $IG$, namely $\mathit{arg max}_{X, t} IG(X, t | \varphi)$.
Intuitively, we aim at maximizing the reduction of weighted average entropy from the parent to the child nodes.
% Maybe a final sentence explaining what this means, information-wise?

\subsection{On Estimating Probabilities}
\label{sec:ProblemSetting.EstProb}

Probabilities and, thus, entropy and information gain are defined for random variables. They are estimated on the subset of the training set $D$ reaching the current node satisfying $\varphi$ by classical frequency counting:
%
\begin{equation}
\label{eq:EstProb}
    \hat{P}(X=t \, | \, \varphi) \equiv \frac{|\{w \in D\ |\ \varphi(w) \wedge w[X] = t\}| }{|\{w \in D\ |\ \varphi(w)| } \approx P(X=t \, | \, \varphi) 
    \, ,\;\;\; 
     \hat{P}(Y=y \, | \, \varphi) \equiv  \frac{|\{w \in D\ |\ \varphi(w) \wedge w[Y] = y\}| }{\{|\{w \in D\ |\ \varphi(w)| } \approx P(Y=y \, | \, \varphi)
\end{equation}
%
where the denominator represents the number of instances $w$ in $D$ that satisfy the condition $\varphi$ (written $\varphi(w)$) and the numerator the number of those instances that further satisfy $X=t$ (resp., $Y=y$).
% \[ P(X=t|\varphi) \approx \frac{i}{n} \quad P(Y=y|\varphi) \approx \frac{j}{n} \]
% where $n$ is the number of the instances in the training set satisfying $\varphi$, and $i$ (resp., $j$) is the number of those instances that further satisfy $X=t$ (resp., $Y=y$).
Frequency counting is supported by the Law of Large Numbers, assuming that the training set is an \textit{i.i.d.} sample from the $P$ probability distribution. Here, the key assumption is that the $P$ probability is the same for the data used for growing the decision tree (the training dataset) and for the data on which the decision tree makes predictions (the test dataset). 

In our scenario, instead, the training dataset belongs to the source domain $D_S$ with probability distribution $P_S$ and the test dataset belongs to the target domain $D_T$ with probability distribution $P_T$, such that $P_T \neq P_S$. To stress this point we use the name \textit{source data} for training data sampled from $D_S$ and \textit{target data} for training data sampled from $D_T$. 
The estimation of probabilities \eqref{eq:EstProb}, and the subsequent estimations of $H$ \eqref{eq:ShannonEntropy} and $IG$ \eqref{eq:BasicIGd}-\eqref{eq:BasicIGc} based on source data can be biased, in statistical terms, relative to the intended target domain. This can result, among other issues, in poor model performance as the trained decision tree classifier will not be suited for the target data.

Formally, for any current path $\varphi$, estimating $\hat{P}(X)$ on $D_S$ implies that it follows the source domain probability distribution: $\hat{P}(X) \sim P_S$. This is also true for $H$ and $IG$ that use the estimated probabilities as well as for the learned classifier built on $IG$. Under covariate shift, we aim for $\hat{P}(X) \sim P_T$ based on the available target domain knowledge to avoid a biased classifier in $D_T$ (recall issue P1 in Section~\ref{sec:ProblemSetting}). This is why in this paper we propose extending the estimated probabilities \eqref{eq:EstProb} by embedding them with target domain knowledge.

% \begin{example}
%     An example here about different estimations based on source and target data.
% \end{example}

% We propose in this paper to extend them by embedding target domain knowledge.

%Algorithmically, the $IG(X, t | \varphi)$ is calculated for all attributes in $\mathbf{X}$ and thresholds

\subsection{Distance between Probability Distributions}
\label{sec:sec:ProblemSetting.DistBtwProbs}

Measuring the distance between the probability distributions $P_S$ and $P_T$ is extremely relevant for detecting distribution shifts. 
We resort to the \textit{Wasserstein distance} $W$ between two probability distributions to quantify the amount of covariate shift and the robustness of target domain knowledge. In the former case, we quantify the distance between $P_S(Y|\mathbf{X})$ and $P_T(Y|\mathbf{X})$. In the latter case, the distance between $P_S(X|\varphi)$ and $P_T(X|\varphi)$. 
We define $W$ between $P_S$ and $P_T$ as:
%
\begin{equation}
\label{eq:WDistance}
    W(P_S, P_T) = \int_{-\infty}^{+\infty} | \mathcal{P}_S - \mathcal{P}_T |
\end{equation}
%
where $\mathcal{P}_S$ and $\mathcal{P}_T$ are the cumulative distribution functions (CDFs) of $P_S$ and $P_T$.\footnote{See \url{https://docs.scipy.org/doc/scipy/reference/generated/scipy.stats.wasserstein_distance.html} for implementation details.} 
% We can interpret \eqref{eq:WDistance} as an optimal transport problem. How much (probability) mass $P_S$ is needed to move from $\mathcal{P}_S$ to construct $\mathcal{P}_T$ at some cost measured by distance. If $\mathcal{P}_S$ to and $\mathcal{P}_T$ are similar, little effort is needed captured by a low distance.

In particular, to address the issue $P_S(\mathbf{X}) \neq P_T(\mathbf{X})$, we need for $P_S(Y|\mathbf{X}) = P_T(Y|\mathbf{X})$ to hold. This equality between the conditional distributions is often assumed but not tested in domain adaptation works. In practice, we want to measure the distance between these two probability distribution using \eqref{eq:WDistance} to insure that our proposed embedding with target domain knowledge is impactful (recall issue P2 in Section~\ref{sec:ProblemSetting}). When this equality is not met, it is difficult to claim that our proposed embedding is addressing the problem of covariate shift. Measuring this distance will allow to evaluate how relaxations of the equality affect the impact of our proposed embedding.

% TODO: move to another file under sections/
\section{Embedding Target Domain Knowledge}
\label{sec:DADT}

When growing a decision tree, the probabilities in \eqref{eq:ShannonEntropy}--\eqref{eq:BasicIGc} are estimated over the training dataset, which is normally a dataset over the source domain. We propose to embed in the estimation some knowledge from the target domain$D_T$, reducing the potential bias in the estimation of the probabilities. There are two probability forms that are to be considered: $P(X=t|\varphi)$  in \eqref{eq:BasicIGd} (resp., $P(X\leq t|\varphi)$ in \eqref{eq:BasicIGc}) and $P(Y=y|\varphi)$ in \eqref{eq:ShannonEntropy}. In fact, the formulas of Entropy and Information Gain only rely on those two forms, and on the trivial relation $P(X\neq t|\varphi) = 1 - P(X=t|\varphi)$ for discrete attributes (resp., $P(X> t|\varphi) = 1 - P(X\leq t|\varphi)$ for continuous attributes).

\subsection{Estimating $P(X=t|\varphi)$}

We assume that some target domain knowledge is available $\hat{P}(X|\varphi)$, possibly for only a few attributes $X$ and/or conditions $\varphi$, which allows us to estimate the target domain marginal probabilities\footnote{Actually, since we consider $x$ in the (finite) domain of $X$ the two forms are equivalent, due to basic identities $P_T(X\leq x|\varphi) = \sum_{X \leq x} P_T(X = x|\varphi)$ and $P_T(X = x|\varphi) = P_T(X\leq x|\varphi) - P_T(X\leq x'|\varphi)$, where $x'$ is the element preceding $x$ in the domain of $X$. Moreover, by definition of conditional probability, we have $P(X=t|\varphi) = P(X=t, \varphi)/P(\varphi)$ and then target domain knowledge boils down to estimates of probabilities of conjunction of equality conditions.}:
%
    \begin{align}
\label{eq:tdk} \hat{P}(X=x|\varphi) \approx P_T(X=x|\varphi) \mbox{\rm\ for $X$ discrete} \quad \hat{P}(X\leq x|\varphi) \approx P_T(X\leq x|\varphi) \mbox{\rm\ for $X$ continuous} 
\end{align}
%
We extend $\hat{P}$ to the case that $\hat{P}(X=x|\varphi)$ is not directly available in the target domain knowledge, by affine combinations for discrete and continuous attributes:
%
    \begin{eqnarray}
\label{eq:aff}
& \hat{P}(X=x|\varphi) = \alpha \cdot  P_S(X=t|\varphi)  + (1-\alpha) \cdot \hat{P}(X=t|\varphi') \\\nonumber
& \hat{P}(X\leq x|\varphi) = \alpha \cdot  P_S(X\leq t|\varphi)  + (1-\alpha) \cdot \hat{P}(X\leq t|\varphi')
\end{eqnarray}
%
%
where $\varphi'$ is a maximal subset of split conditions in $\varphi$ for which $\hat{P}(X=t|\varphi')$ is in the target domain knowledge, and $\alpha \in [0, 1]$ is a parameter to be set. In particular, setting $\alpha=0$ boils down to estimate probabilities based on the source data only.
%
With such assumptions, $P(X=t|\varphi)$ in \eqref{eq:BasicIGd} (resp., $P(X\leq t|\varphi)$ in \eqref{eq:BasicIGc}) can be computed from the target domain knowledge as $P(X=t|\varphi) = \hat{P}(X=t|\varphi)$ (resp., $P(X\leq t|\varphi) = \hat{P}(X \leq t|\varphi)$). 


\subsection{Estimating $P(Y=y|\varphi)$}

Let us consider the estimation of $P(Y=y|\varphi)$ in \eqref{eq:ShannonEntropy} over the target domain. It is legitimate to ask whether, under the assumption of covariate shift, that is the same probability as in the source domain. 
%
The answer is negative. Covariate shift states that $P_S(Y|\mathbf{X}) = P_T(Y|\mathbf{X})$, namely that the probability mass function of $Y$ conditional to fixing \textit{all of the} variables in $\mathbf{X}$ is the same in the source and target domains. Formally, covariate shift assumes:
%
    \begin{align}
\label{eq:covshift}
 \forall \mathbf{x} \in \mathbf{X}. \forall y \in \mathbf{Y}. \ P_S(Y=y|\mathbf{X=x}) = P_T(Y=y|\mathbf{X=x})
\end{align}
%
However, this does not necessarily imply $P_T(Y=y|\varphi) = P_S(Y=y|\varphi)$ for a current path $\varphi$.

\begin{example}
Let $\mathbf{X} = X_1, X_2$ and $Y$ be binary variables, and $\varphi$ be $X_1=0$. Since
$P(X_1, X_2, Y) = P(Y|X_1, X_2) \cdot P(X_1, X_2)$, the full distribution can be specified by stating $P(Y|X_1, X_2)$ and $P(X_1, X_2)$. Let us consider any distribution such that:
\[P_S(X_1, X_2) = P_S(X_1) \cdot P_S(X_2) \quad P_T(X_1=X_2)=1 \quad Y = I_{X_1=X_2} \]
i.e., $X_1$ and $X_2$ are independent in the source domain, while they are almost surely equal in the target domain. Notice that $Y = I_{X_1=X_2}$ readily implies that $P_S(Y|X_1, X_2) = P_T(Y|X_1, X_2)$, i.e., the covariate shift condition (\ref{eq:covshift}) holds. Using the multiplication rule of probabilities, we calculate:
\[ P_S(Y|\varphi) = P_S(Y|X_1=0) = P_S(Y|X_1=0, X_2=0) \cdot P_S(X_2=0|X_1=0) + P_S(Y|X_1=0, X_2=1) \cdot P_S(X_2=1|X_1=0) =\]
\[ = P_S(Y|X_1=0, X_2=0) \cdot P_S(X_2=0) + P_S(Y|X_1=0, X_2=1) \cdot P_S(X_2=1) \]
where we exploited the independence of $X_1$ and $X_2$ in the source domain, and
\[ P_T(Y|\varphi) = P_T(Y|X_1=0) = P_T(Y|X_1=0, X_2=0) \cdot P_T(X_2=0|X_1=0) + P_T(Y|X_1=0, X_2=1) \cdot P_T(X_2=1|X_1=0) =\]
\[ =  P_T(Y|X_1=0, X_2=0)\]
were we exploited the equality of $X_1$ and $X_2$ in the target domain.
$P_S(Y|\varphi)$ and $P_T(Y|\varphi)$ are readily different when setting $X_1, X_2 \sim Ber(0.5)$ because $P_S(Y=1|\varphi) = 1 \cdot 0.5 + 0 \cdot 0.5 \neq 1 = P_T(Y=1|\varphi)$. 
\end{example}

By abstracting from the example, we rewrite $P_T(Y=y|\varphi)$ as follows:
%
    \begin{align}
\label{eq:rewry}
P_T(Y=y|\varphi) =  \sum_{\mathbf{x} \in \mathbf{X}} P_T(Y=y|\mathbf{X}=\mathbf{x}, \varphi) \cdot P_T(\mathbf{X}=\mathbf{x}|\varphi) = \sum_{\mathbf{x} \in \mathbf{X}} P_S(Y=y|\mathbf{X}=\mathbf{x}, \varphi) \cdot P_T(\mathbf{X}=\mathbf{x}|\varphi) 
\end{align}

where the final equation exploits the covariate shift assumption. (\ref{eq:rewry}) rewrites $P_T(Y=y|\varphi)$ in terms of probabilities over the source domain, namely $P_S(Y=y|\mathbf{X}=\mathbf{x}, \varphi)$, and target domain knowledge, namely $P_T(\mathbf{X}=\mathbf{x}|\varphi)$.
However, varying $\mathbf{x}$ over all possible combination of values of $\mathbf{X}$ is not feasible, as it would require extensive target domain knowledge to estimate $P_T(\mathbf{X}=\mathbf{x}|\varphi)$ for all combinations $\mathbf{x} \in \mathbf{X}$. This would be an issue also in the case we had a full sample of the target domain, as it would require the sample to be large enough for observing each value $\mathbf{x} \in \mathbf{X}$.
Thus, we choose to vary values w.r.t. a single attribute $X_w$ and define the estimate:
%
\begin{align}
\label{eq:wpyphi}
\hat{P}(Y=y|\varphi) = \sum_{x \in X_w} P_S(Y=y|X_w=x, \varphi) \cdot \hat{P}(X_w=x|\varphi) 
\end{align}
where we use now target domain knowledge
about $P_T(X_w=x_w|\varphi)$. The attribute $X_w$ is chosen such that the summation is close to the estimand $P_T(Y=y|\varphi)$. However, such an attribute $X_w$ may depend on the current path $\varphi$,
which would require target domain knowledge on the conditional distribution of $Y$. Thus, we only consider $\varphi = true$, and then choose $X_w$ such that:
%
\begin{align}
\label{eq:wpy}
X_w = arg min_{X} W( \hat{P}^X(Y), P_T(Y) ) \quad \mbox{\rm where\ } \hat{P}^X(Y) = \sum_{x \in X} P_S(Y=y|X=x) \cdot P_T(X=x) 
\end{align}
namely, such that the distance between estimated and target domain marginal probability of $Y$ is minimal. In terms of target domain knowledge, this requires to know the (unconditional) distribution of the class in the target domain. 

\subsection{How Much Target Domain Knowledge}

We can now formalize the range of cases described in Section \ref{sec:problemstatement}.

\smallskip
\textit{\textbf{No target domain knowledge.}} This amounts at having no $\hat{P}$ available. This means that $\hat{P}(X=x|\varphi) = P_S(X=x|\varphi)$, i.e. $\alpha=0$ is necessarily set in (\ref{eq:aff})), and, whatever $X_w$ is, $\hat{P}(Y=y|\varphi) = P_S(Y=y|\varphi)$. In summary, the estimations boil down to growing the decision tree using the source data without any modification.

\textit{\textbf{Full target domain knowledge.}} We assume to have target domain knowledge for all attributes, i.e., $\alpha=1$ is  set in (\ref{eq:aff})), and to know which attribute $X_w$ minimizes (\ref{eq:wpy}).

\smallskip
The full target domain knowledge is the strongest possible assumption within our approach, but not in general. We set then an additional baseline.

\textit{\textbf{Target-to-target baseline.}} In this scenario, the decision tree is grown on the target data. Such a scenario does not require covariate shift, since probabilities $P(X=t|\varphi)$ and $P(Y=y|\varphi)$ are estimated directly over the target domain. 

\smallskip
Finally, between the no target domain and the full target domain knowledge there are a number of intermediate scenarios based on the amount of available target domain knowledge:

\begin{itemize}
    \textcolor{red}{\item tba}
\end{itemize}


\newpage
\section{Experiments}
\label{sec:Experiments}

We report here experiments on real and synthetic datasets.

\subsection{ACSIncome dataset}

Let us consider the \textit{ACSPublicCoverage} dataset  -- an excerpt of the 2017 U.S. Census data \cite{dingRetiringAdultNew2021} which provides the same feature sets for different geographical regions (American states), which may have different distributions. This allows us to examine the impact of our method given a wide range of distribution shifts. We utilize the prediction task, constructed by the dataset creators, of whether or not a low income person has public medical coverage.. Unless otherwise stated, we consider the attributes: SCHL, MAR, AGEP, SEX, CIT, RAC1P, with AGEP continuous and all other discrete. \textcolor{red}{more extensive description of attributes. Explain prediction task (is it really Income?? or Coverage)}
 
\begin{figure}[t]
  \centering
  \includegraphics[width=0.51\linewidth]{img/fig1.png}\hspace{0.8cm}
  \includegraphics[width=0.40\linewidth]{img/fig2acc.png}
  \caption{TBD}\label{fig:srtg}
\end{figure}

We consider pairs of source and target datasets consisting of data from different U.S. states. A decision tree is trained on 75\% of source data, and tested on 25\% of the target data. Stopping criteria include the following: a node must have at least 5\% of the training data, and not all instances have the same class value (purity level set to 100\%), the maximum tree depth is 8.

\subsection{Covariate Shift Assumption}
\label{sec:Experiments.CovariateShift}

The scatter plot Fig. \ref{fig:srtg} (left) relates the Wasserstein distances for each attribute and source-target pair. On the x-axis, there is the distance between the
marginal attribute distributions, i.e., $W(P_S(X), P_T(X))$. On the y-axis, there is the distance between the target and estimated marginal class distribution, i.e.,$W( \hat{P}^X(Y), P_T(Y) )$ from (\ref{eq:wpy}). Marginal attribute distributions are rather small, with the exception of CIT and RAC1P which have more variability.  The distances between target and estimated class distributions is instead much larger, for all attributes. Interestingly, the plot shows that the \textit{ACSIncome} dataset does not in general satisfy the covariate shift assumption (at least for marginal distributions), but rather the opposite: close attribute distributions and distant conditional class distributions. This fact will help us in exploring how much our approach relies, in practice, on the covariate shift assumption.

\textit{\textbf{No target domain knowledge vs target-to-target baseline.}} Let us consider the scenario of no target domain knowledge, i.e., training a decision tree on the source training data and testing it on the target test data. We compare the decision tree accuracy in this scenario (let us call $ACC_{ntdk}$) to the accuracy of training a decision tree on the target training data and testing on the target test data ($ACC_{tt}$), a.k.a., the target-to-target baseline. Recall that accuracy estimates on a test set (of the target domain) the probability that the classifier prediction $\hat{Y}$ is correct w.r.t. the ground truth $Y$:
%
\[ ACC = P_T(\hat{Y}=Y) \]
%
The heat-map plot Fig. \ref{fig:srtg} (right) shows for each source-target pair of states the absolute difference in accuracy $ACC_{ntdk}-ACC_{tt}$ between the target-to-target baseline and the no target domain knowledge scenario. In most of the cases the difference is negative, meaning that there is an accuracy loss in the no target domain knowledge scenario. \textcolor{red}{to describe the states with an increase}
 
\begin{figure}[t]
  \centering
  \includegraphics[width=0.50\linewidth]{img/fig3acc.png}\hspace{0.8cm}
  \includegraphics[width=0.43\linewidth]{img/fig4acc.png}
  \caption{TBD}\label{fig:res}
\end{figure}


\textit{\textbf{Full target domain knowledge vs No target domain knowledge.}} Let us consider now target domain knowledge. $P_T(X=t|\varphi)$ and 
$P_T(X\leq t|\varphi)$ are calculated from the target (training) data, for each $X$, $t$, and $\varphi$ -- which amounts at the full target domain knowledge scenario. The decision tree in this scenario is grown on the source (training) data but probabilities are estimated by full target domain knowledge using (\ref{eq:tdk}), and (\ref{eq:aff}) with $X_w$ minimizing (\ref{eq:wpyphi}).

Let us compare the accuracy of the decision tree grown using full target domain knowledge (let us call it $ACC_{ftdk}$) to the one with no target domain knowledge ($ACC_{ntdk}$). 
%
In 45\% of the source-target pairs, 
the accuracy of the full target domain knowledge scenario is better than the one of the no target domain knowledge scenario ($ACC_{ftdk} > ACC_{ntdk}$), and in 24\% of the pairs they are equal ($ACC_{ftdk} = ACC_{ntdk}$).
%
This gross comparison needs to be investigated more in depth. Let us define the relative gain in accuracy as:
\[ rACC = \frac{ACC_{ftdk}-ACC_{ntdk}}{|ACC_{tt}-ACC_{ntdk}|} \cdot 100 \]
where $ACC_{tt}$ is the accuracy in the targe-to-target baseline. The relative gain quantifies how much of the loss in accuracy in the no target domain knowledge scenario has been recovered in the full target domain knowledge scenario. The absolute value in the denominator is intended to cover the cases where $ACC_{ntdk} > ACC_{tt}$. Moreover, to prevent outliers due to very small denominators, we cap $rACC$ to the $-100$ and $+100$ boundaries. The mean value of $rACC$ over all source-target pairs is $10.5$, i.e., on average our approach recover 10.5\% of the loss in accuracy. However, there is a large variability, which we examine further in the next section.

\subsubsection{Covariate Shift}
(add covariate shift section above here?)
We test whether the difference in.. is due to the fact that different pairs match or do not match the covariate shift assumption. In order to quantify the covariate shift, we define specifically for a decision tree $T$:
%
\begin{align}
\label{eq:wtree}
W(T) = \sum_{\varphi\ \mbox{\rm path of a leaf of\ } T} W( \hat{P}(Y|\varphi), P_T(Y|\varphi)) \cdot P_T(\varphi)
\end{align}
as the average  Waisserstain distance between the estimated and target domain class distributions at leaves of the decision tree, weighted by the leaf probability in the target domain. We write $W(T_{ntdk})$ and $W(T_{ftdk})$ respectively for denoting the amount of covariate shift for the decision tree grown in the no target domain knowledge and with full target domain knowledge scenarios.
%
The scatter plot Fig. \ref{fig:res} (left) shows the relative accuracy (in color) at the variation of $W(T_{ntdk})$ and $W(T_{ftdk})$\footnote{$W(T_{ntdk})$ and $W(T_{ftdk})$ appear to be correlated. While they are specific of their respective decision trees, they both depend on the distribution shift between the source and target domain.}.
We make the following qualitative observations:
\begin{itemize}
    \item when $W(T_{ftdk})$ is small, say smaller than $0.05$, i.e., when the covariate shift assumption holds, the relative accuracy is high, i.e., using target domain knowledge allows for recovering the accuracy loss;
    \item when $W(T_{ftdk})$ is large, say larger than $0.10$, then the relative accuracy is low or even negative. Interestingly, a pattern with very low $rACC$ is highlighted by the red points shown for $W(T_{ftdk})$ smaller than $W(T_{ntdk})$. This can be motivated by the fact that \textcolor{red}{to be continued}
\end{itemize}
Let us consider now how to determine quantitatively on which pairs there is a large relative accuracy.
Fig. \ref{fig:res} (right) reports the mean $rACC$ for source-target pairs sorted by the difference distances. Ordering by $W(T_{ftdk})$ allows to identify source-target pairs for which our approach works the best, followed by ordering by $W(T_{ntdk})$ and by the marginal distance between $P_T(Y)$ and the estimation $\hat{P}^{X_w}(Y)$ using the attribute $X_w$ from (\ref{eq:wpy}). We observe that:

\begin{itemize}
    \item $W(T_{ftdk})$ and $W(T_{ntdk})$ are difficult to be estimated, as they would require target domain knowledge $P_T(Y|\varphi)$ for each\footnote{Or, at least, for the leaves with the largest target domain probability $P_T(\varphi)$.} leaf in $T_{ftdk}$ and $T_{ntdk}$ respectively.
    \item the distance $W(\hat{P}^{X_w}(Y), P_T(Y))$ is easier to calculate/estimate, as it regards only the marginal distribution $P_T(Y)$ and the marginal conditional distributions $P_T(Y|X)$ in (\ref{eq:wpy}). These two distributions can be estimated e.g., by collecting a relative small sample of instances over the target domain.
\end{itemize}

\begin{figure}[t]
  \centering
  \includegraphics[width=0.50\linewidth]{img/fig3dp.png}\hspace{0.8cm}
  \includegraphics[width=0.43\linewidth]{img/fig4dp.png}
  \caption{TBD}\label{fig:resdp}
\end{figure}

\subsection{ACSIncome dataset: additional experiments}
\label{sec:introduction}

\textbf{Fairness metric: demographic parity.}
Other quality metrics beyond accuracy can degrade in presence of covariate shift. We consider here the fairness metric of demographic parity, referred to the protected attribute SEX. Demographic parity quantifies the disparity between predicted positive rate for men and women: 
\[ DP = |P(\hat{Y}=1|\mbox{SEX=women})-P(\hat{Y}=1|\mbox{SEX=men})| = \]
The lower the $DP$ the better is the fairness performance.
Fairness-aware classifiers control for demographic parity. We use here a classifier-agnostic post-processing method that specializes the decision threshold for each protected group \cite{hardtEqualityOpportunitySupervised2016a}. The correction is applied after the decision tree is trained. We can mimick the reasoning done for the accuracy metric, and introduce relative demographic parity:
\[ rDP = \frac{DP_{ntdk}-DP_{ftdk}}{|DP_{tt}-DP_{ntdk}|} \cdot 100 \]
where at the numerator the two terms are swapped because improvement consists of lowering the $DP$. The mean value of $rDP$ over all source-target pairs is 37, meaning that on average our approach recover 37\% of the loss in demographic parity. Fig. \ref{fig:resdp} is the analogous of Fig. \ref{fig:res} for relative demographic parity. Considerations similar to the case of the accuracy metric apply, but not exactly the same. While distance between $\hat{P}(Y|\varphi)$ and $P_T(Y|\varphi)$ at leaves with path $\varphi$ is an appropriate choice when considering accuracy (which relies on the most likely class value), it is only partly appropriate when considering demographic parity. In fact, if $\hat{P}(Y|\varphi, \mbox{\rm SEX=male})$ and $P_T(Y=1|\varphi, \mbox{\rm SEX=male})$ are distant, and  $\hat{P}(Y|\varphi, \mbox{\rm SEX=female})$ and $P_T(Y=1|\varphi, \mbox{\rm SEX=female})$ are also distant, but the differences of those probabilities are close, then the demographic parity metric is low. Intuitively, errors that are common to male and female are fine for demographic parity, but not for accuracy. As a consequence, $W(T_{ntdk}$ and $W(T_{ntdk}$ are not the best distances to analyze the $rDP$. In fact, Fig. \ref{fig:resdp} (left) shows a less clear winner for low values of the axes. Moreover, Fig. \ref{fig:resdp} (right) shows that the distance $W(\hat{P}^{X_w}(Y), P_T(Y))$ is a better way of selecting pairs over which our approach works best.
 
Can we relate the impact of our intervention on DP

\textcolor{red}{TBA: experiment with partial target domain knowledge (e.g., $\varphi$ with at most 2 or 3 split conditions).}

\medskip

\textcolor{red}{TBA: experiment with noisy target domain knowledge, and setting $\alpha$ to control for noise.}

\medskip
\textcolor{red}{TBA: experiment with data with more attributes, but target domain knowledge only on a subset of them.}


\subsection{Synthetic dataset}
\label{sec:Experiments.SyntheticDataset}


TBA

\section{Discussion and future work}
\label{sec:Discussion}




\subsection{Conclusion}
\label{sec:Conclusion}




==> previous_version/OurApproach.tex <==
%
We present the domain-adaptive weight modification for $IG$ that, in turn, gives way to the \textit{domain-adaptable information gain} ($DIG$) split criterion. We define $DIG$ in its most general form as:
%
\begin{equation}
    \label{eq:BasicDIG}
    DIG(\varphi, X) = H(\varphi) - \sum_{x \in X} \Psi_D(x) H (\varphi| x)
\end{equation}
%
where $\Psi_D(x)$ represents the domain-adaptive weight over the domain space $D=D_S \times D_T$, replacing the inherent weight $P(x)$ in \eqref{eq:BasicIG}.

We interpret $\psi_D(x)$ in \eqref{eq:BasicDIG} as the probability of $x$ occurring given the functional form $\psi$, which maps the event of interest over the domain space $D$. It, thus, weights the event-specific conditional entropy contributions $H(\varphi|x)$ onto the overall conditional entropy $H(\varphi|X)$ based on $D$, meaning on either elements of $D_S$ or $D_T$ or both. We want $\psi_D$ to behave like probability. From this last property, we want the domain-adaptive weight to follow the target domain distribution or a resulting distribution based on it. 
% Therefore,

{\bettina Why did you change from Psi to psi?}

{\bettina The para is a bit strange: You start by sayin that you interpret psi as the probability of ..., and then later on you say that you want psi to behave like probability. Better streamline this.}

\subsection{Proposed domain-adaptive weight}
\label{sec:OurApproach.Lambda}

For $DIG$ \eqref{eq:BasicDIG}, we define the \textit{domain-adaptive weight} $\psi_D$ as:
%
\begin{equation}
    \label{eq:lambda}
    \psi_D(x) = \lambda \times P_S(x) + (1 - \lambda) \times P_T(x)
\end{equation}
%
where $\lambda \in [0, 1]$ is a \textit{tuning parameter} that allows us to switch between the source $P_S$ and target $P_T$ domain distributions for obtaining the probability of the event $x \in X$. 

Under \eqref{eq:lambda}, we have three scenarios: $\psi_D(x) \sim P_S$ when $\lambda=1$; or $\psi_D(x) \sim P_T$ when $\lambda=0$; or $\psi_D(x) \sim P_S \cap P_T$ when $\lambda \in (0, 1)$. 
{\bettina Can you intersect two probability (distributions)? (Sorry, I may be missing something here.)}
Clearly $\psi_D(x) \in [0, 1]$ for all values of $\lambda$ as $P_S(x), P_T(x) \in [0, 1]$. Do notice that when $\lambda=1$, $DIG$ \eqref{eq:BasicDIG} becomes $IG$ \eqref{eq:BasicIG}. Hence, $IG$ is contained in $DIG$. When we estimate \eqref{eq:BasicDIG}, while $H(\varphi)$ is solely constructed on the source domain, $H(\varphi|X)$ can use elements from either or both source and target domains based on $\lambda$.

We choose this functional form for its simplicity as we only need access to the target probability of $P_T(x)$ and $\lambda$. $DIG$ is an \textit{in-processing step}. Two factors are important to consider for realistically implementing any form of $\psi_D$. First, the split criterion is called recursively when growing the decision tree and, at each time, conditional on the current path $\varphi$. Second, access to the target domain tends to be limited in practice and we might not be able to draw all target probabilities $P_T(x)$ to match each $P_S(x)$. For these reasons, a simple functional form as the one proposed \eqref{eq:lambda} is appealing. 
%For instance, we could use some distance measure $d$ instead of $\lambda$ for mixing the probabilities, but it would require defining $d$. 
Other functional forms are possible for $DIG$, which can be explored in subsequent works. Overall, we see \eqref{eq:BasicDIG} as a blueprint for domain-adaptive decision trees: the goal here is to showcase its potential for reaching fairer decision tree classifiers.

Let us rewrite $DIG$ \eqref{eq:BasicDIG} with the proposed $\psi_D$ \eqref{eq:lambda}:
% %
% \begin{equation}
%     \label{eq:OurDIG}
%     DIG(\varphi, X, \lambda) = H(\varphi) - \sum_{x \in X} \big( \lambda \times P_S(x) + (1 - \lambda) \times P_T(x) \big) H (\varphi| x)
% \end{equation}
% %
%
\begin{align}
\label{eq:OurDIG}
    DIG(\varphi, X, \lambda) 
    = {} & H(\varphi) - \sum_{x \in X} \big( \lambda \times P_S(x) + (1 - \lambda) \times P_T(x) \big) H (\varphi| x) \\
    = & \sum_{x \in X} - P_S(x) \log_2(P_S(x)) \; - \nonumber\\
    & \;\;\; \sum_{x \in X} - \big( \lambda \times P_S(x) + (1 - \lambda) \times P_T(x) \big) P_S(\varphi|x) \log_2(P_S(\varphi|x)) \nonumber
\end{align}
%
where we include $\lambda$ as a parameter for the split criterion. In the second line, using the definition of (Shannon's) entropy \eqref{eq:ShannonEntropy}, we write out the entropy terms based on their domains.
% As with $IG$, it is also a random variable. Depending on $\lambda$, it can follow either the source or target domain or a mixture of both. 
In the next sections, we look further into the key elements of $DIG$ \eqref{eq:OurDIG}: $P_T(x)$ (Section~\ref{sec:OurApproach.ExternalKnowledge}) and $\lambda$ (Section~\ref{sec:OurApproach.NoSurprises}).

{\bettina I didn't check the formula}

\subsection{External Knowledge}
\label{sec:OurApproach.ExternalKnowledge}

In practice, \eqref{eq:OurDIG} is estimated using the corresponding \textit{empirical probabilities}: $\hat{P}_S(\varphi)$, $\hat{P}_S(\varphi|x)$, $\hat{P}_S(x)$, and $\hat{P}_T(x)$. These estimates are derived from the frequencies of realizations in the training data when learning the decision tree classifier.\footnote{
Recall,
\begin{equation*}
    \hat{P}(x) = \sum_{i} \frac{f_i(X)}{|X|}
\end{equation*}
where $f_i(X) = |\{ x \in X \; : \; X[i] = x\}|$ is the number of instances from $X$ with class $x$ and $|X|$ the number of classes that constitute the attribute $X$.}
We note that this \textit{naive estimation procedure} for Shannon's entropy has been shown to have a downward bias \cite{Schurmann_2004}. New estimates have been specifically proposed for addressing the biased estimators in the context of decision tree learning, though with marginal gains in terms of model performance \cite{DBLP:conf/icml/Nowozin12}, which might explain why the literature still relies on the naive estimator for entropy. We too rely on the naive estimator, 
but
%BB though 
acknowledge that future work on the theoretical properties of our proposed domain-adaptive weight can be of interest. See Appendix~\ref{appendix:EstimationBiasEntropy} for details on this estimation bias.

All probabilities but $\hat{P}_T(x)$ can be estimated using the source data $\mathcal{D}_S \in D_S$. For said probability, we use the target data $\mathcal{D}_T \in D_T$ for which, based on our selection bias scenario, we have limited access. There are two points to consider regarding $\mathcal{D}_T$. First, we need to define what we consider as \textit{outside information} for deriving $\hat{P}_T(x)$. Here, we focus on cases of \textit{tabular data}, but remark that other forms of representation are possible. For example, we could use logic-based inference or a human expert to obtain the target weights. Second, we need to keep in mind that such probabilities are \textit{defined dynamically while growing the decision tree}, i.e., conditional on $\varphi$. 
{\bettina exactly. And that gets lost a bit through the notation earlier.}
We cannot determine them statically and then feed them to the decision tree learning algorithm. The chosen external knowledge representation must be able to change according to $\varphi$. 

Given these two points, the tabular data for the external knowledge needs to mirror the data structure of the source data. In other words, it needs to provide information on the $\mathbf{S}$ $m$ sensitive and $\mathbf{X}$ $p$ non-sensitive attributes contained in $\mathcal{D}_S$
{\bettina weird grammar. proposal, pls check:
$\mathbf{S}$, the $m$ sensitive attributes, and $\mathbf{X}$, the $p$ non-sensitive attributes, contained in $\mathcal{D}_S$
}
so that for any possible current path $\varphi$, it can provide a $\hat{P}_T(x)$. In an ideal situation, we have access to $\mathcal{D}_T$ such that it fully mirrors $\mathcal{D}_S$. In practice, this is usually not the case and we use other sources of information to complement or even replace $\mathcal{D}_T$. In this paper, we resort to using \textit{official statistics} derived by governments from census data. 

{\bettina This comes rather out of the blue and ends up a bit "buried". Could you preview this earlier?}

For instance, suppose we find ourselves at the current node based on $\varphi=\{ \text{(Gender, female), (Employed, yes)} \}$ and we are considering the split candidate \texttt{Income} and its threshold value \texttt{> 50000}, meaning that we are looking at ``individual instances that identify as female, are employed, and earn more than 50000 euros''. Ideally, the external knowledge representing the target domain, $\mathcal{D}_T$ contains the columns for the attributes \texttt{Gender}, \texttt{Employment}, and \texttt{Income} and we are able to query this data using $\varphi$ plus the split candidate. We then obtain $\hat{P}_T(x)$ in \eqref{eq:OurDIG} by calculating the proportion of employed females earning more than 50000 euros in $\mathcal{D}_T$. However, we probably are in the situation where we do not have a full dataset of that kind and, thus, we need to approximate the current path with the split candidate from other sources. What this means, in practice, is that we might have to preemptively prepare for these potential splits and, at least, provide a default value in case the considered split is not contained in the external knowledge.  

Formally, we define the \textit{external knowledge} $\mathcal{D}_T$ as $\{p^*_1, p^*_2, \dots, p^*_k\ \; | \; \varphi \}$ where $p^*_k=P^*(X_k=x_k) \sim \mathcal{P}_T(\mathbf{X})$ such that the $k$ frequency corresponds to the $k$ attribute in $\mathcal{D}_S$ under the current path $\varphi$. We explore the different ways we handle $\mathcal{D}_T$ when we discuss the learning of the domain-adaptive tree. 

{\bettina k-th (sorry, superscripts don't work in this Latex environment) ?}

\subsection{Fairness as No Surprises}
\label{sec:OurApproach.NoSurprises}

{\bettina I must say that the "no surprises" idea doesn't help me understand what's going on, and I also struggle to link "surprise" to "fairness". I believe that we essentially mean the same when we talk about "surprise" (Jose and Kristen) and when we talk about "visibility" (Bettina); but I believe the visibility idea is more entrenched in the fairness literature. Maybe we should discuss this once more.}

Is there a fairness interpretation to the proposed domain adaptive weight \eqref{eq:lambda} and, in turn, to the resulting $DIG$ \eqref{eq:OurDIG}? Our view here is based on the notion of \textit{low entropy as no surprises} (Section~\ref{eq:ShannonEntropy}), and on Tversky and Kahneman's interpretation \cite{tversky_judgment_1974} of \textit{probabilities as statements of an event $x$'s representativeness regarding the class $X$ it belong to}. We consider the misrepresentation of the target data, due to selection bias, as a source of unfairness when growing a decision tree classifier due to the uncertainty it introduces when evaluating a splitting candidate.

To illustrate our point, suppose we are considering \texttt{Gender} as the splitting candidate $X$ where $x$ can equal \texttt{female} or \texttt{male}. Further, suppose females represent 30\% of the source population but an even 50\% of the target population. 
{\bettina You are looking at unconditional probabilities of gender here - does that mean your example takes place at the root node?}
Both proportions are 
%BB Each proportions are, respectively, 
captured by the datasets and their domain-specific distributions: $\mathcal{D}_S \sim P_S$ and $\mathcal{D}_T \sim P_T$. Under \eqref{eq:OurDIG} with an $\lambda=1$ (i.e., a standard $IG$), when learning the decision tree the contribution to the  conditional entropy $H(\varphi \; | \; \text{\texttt{Gender}})$ will be: $0.7 \times H(\varphi \; | \; \text{\texttt{male}})$ and $0.3 \times H(\varphi \; | \; \text{\texttt{female}})$. This is an issue when we consider that our target population is evenly split over \texttt{Gender}, meaning that we are growing a decision tree that weights the male informational contributions higher to be deployed on a population where male and females have the same informational contributions. Here, $P_S(x)$ mis-represents $P_T(x)$, 
{\bettina please use uniform spelling: misrepresent or mis-represent}
which is an issue as this weight conditions how the tree continues to grow beyond $X$. In terms of entropy, the learned decision tree 
expects
%BB is expecting 
to be surprised by a female instance based on the source population 
{\bettina do you mean "expects to be surprised" because the 30 percent is rarer than an "unsurprising" 50 percent?}
and will, thus, misjudge the certainty 
{\bettina the certainty? not the probability?}
of the event \texttt{female} when used on the target population.

Given $\mathcal{D}_T$, we can address this problem when learning the classifier under $DIG$ \eqref{eq:OurDIG} by relaxing $\lambda$ away from 1. Then the weight for the informational contribution of female instances will increase relative to the male instances, and the split decision will approximate the target population. In that sense, the weight, or probability, is more representative of the class \texttt{Gender} in the target domain as it reflects how its instances, or events, are distributed. As the weight becomes more representative, the possibility for surprises diminishes as the decision tree 
already incorporates
%BB is already incorporating 
the correct information. In doing so, this reduces the chances for the decision tree to misclassify female instances on the target population and, thus, reduce the potential for unfair decision-making. This also, in turn, reduces the possibility of a 
poorly-performing
%BB poor-performing 
model on the target population.



% Consider gender, population-wise $p_i=\frac{1}{2}$, so in theory $H(gender)$ would be the same in Pisa and in Prato. But what if Pisa has 70\% females while Prato only 55\%? Since it's more likely to find a female in Pisa and thus predict her (i.e., no surprises): H(gender|D=Pisa) < H(gender|D=Prato), no? \textit{We want $H$ to reflect surprises in going from the source to the target!}

\subsection{Learning a (Fairer) Domain-Adaptive Decision Tree}

\textcolor{red}{-- -- -- you are here -- -- --}

- write the algo for learning dt

- write algo for gettargetp

- write implementation specific parts (or more on experiemnts)

\begin{algorithm}
\caption{LearnTargetRepresentativeTree}
\label{alg:RepTree}
\begin{algorithmic}[1]

\Require $\mathcal{D}$, $EK$, $\lambda$
\Ensure{$|EK| \neq \emptyset $ and $\lambda \in [0, 1]$}

\vdots

\end{algorithmic}
\end{algorithm}

% \subsection{On Missing External Knowledge}

% \ja{ TBD later: unclear to me how to proceed here. Also, this in itself (as discussed this week) can become a separate paper. This to be seen when we go over the experiments \dots}

% \subsection{Theoretical Section about the Change in Lambda}
% What do we expect to be the impact on predictions as lambda moves from zero (no intervention) to one (outside information is used for 100 percent of information gain calculation?
% \par{Intuition} Taking up the example of a store stocking or not stocking female football shoes, let's state our intuition of the impact of increasing Lambda. Say a store is using customer data is to predict whether each customer is likely to purchase various styles of football shoe, and that these predictions will determine how many of each size and style of shoes the store will stock. 

% We imagine a case where the customer data contained a much lower-than-population number of women, but that those women did buy football shoes at a rate similar to (at least not way lower than) male customers (a reasonable hypothetical for a sports supplies store). Note that in this case we have no special knowledge of the rate of Y in the target domain (ie the rate that females in the population as a whole do or would by football shoes). In fact, thought data on this may be available, we know that it may in fact be impacted by the very issue we are trying to deal with (how often women's football shoes are made available to or presented as an option for women).

% In this case, a lambda of zero we would expect that an accurate classifier would predict that women's shoes should be stocked at a low rate, one that reflects the amount of shoes that their low number of female customers buy (even if female customers buy football shoes at a high rate).

% An increase in lambda is expected to increase the stocking of football shoes in women’s sizes, but why? It would impact whether or not it split on gender and this would do what?

%
% EOS
%


==> previous_version/ProblemSetUp.tex <==
%
We cover the necessary background while motivating the proposed domain-adaptive weight modification to the information gain split criterion. {\bettina Strange intro sentence - sounds like a meta-summary of this section? Please check whether this was some left-over from a sketch stage.} We assume a scenario in which the available training population (\textit{source domain} $D_S$) is not representative of the intended test population (\textit{target domain} $D_T$). We also assume to have ample access to information from $D_S$, but limited access to information from $D_T$. {\bettina What does that mean? What kind of information?} We use uppercase letters for random variables and lowercase letters for their assignments. Let $\mathbf{S} \in {\rm I\!R}^{m}$ denote the set of $m$ \textit{sensitive attributes} and $\mathbf{X} \in {\rm I\!R}^{p}$ denote the set of $p$ \textit{non-sensitive attributes}.
% , where attributes in either set can be discrete or continuous. 
Finally, let $Y \in \{-, +\}$ denote the \textit{ground-truth
%%BB groundtruth 
class} and $\hat{Y}$ its corresponding \textit{predicted class} to be determined by the classifier.

{\bettina General Q: is the notion of (non-)sensitive attributes well-known enough, especially in an interdisciplinary setting like this one? Maybe there should be one more sentence to explain it?}

\subsection{Selection Bias under Domain Adaptation}
\label{sec:sec:ProblemSetting.SelectionBias}

Often the \textit{source data} $\mathcal{D}_S \in D_S$ used for training the classifier misrepresents the \textit{target data} $\mathcal{D}_T \in D_T$ due to selection bias \cite{Heckman_sample_1976}. Selection bias occurs when there exists some \textit{(self-)selection mechanism} $\zeta$ that determines the constitution of $\mathcal{D}_S$ non-randomly \cite{Heckman_sample_1979}. Selection bias violates the standard \textit{i.i.d.} assumption as only selected instances, $\zeta = 1$
{\bettina A mechanism (above) is a scalar (here)?}%
, are recorded in $\mathcal{D}_S$, meaning that generalizations from the source to the target domain are no longer trivial. It helps to picture this problem as one of \textit{missing information} in which the classifier cannot learn from those data instances unavailable to it due to $\zeta$ \cite{Cortes2008_SampleSelectionBias}. 
{\bettina General question: Is this really necessarily selection bias? If we collect data from two states, and in the first, there are 30\% women and in the other one 60\% women, then this could just be perfectly accurate demographics of the two states, with no bias at all in the sampling in either state. Calling this a selection bias assumes some weird position in which the demographics of one state become the normative truth. (The 3rd sentence in Section 4.3 suggests this interpretation.) }


We tackle selection bias as a domain adaptation problem. In practice, models struggle to generalize outside their training setting. Beyond poor performance, this issue can have serious fairness consequences as deployed models can be oblivious to their new setting and perpetuate potential biases (recall, e.g., Amazon's sexist hiring algorithm \cite{DastinAmazonSexist}). Domain adaptation, a subset of transfer learning, studies how to achieve robust models when the training ($\mathcal{D}_S$) and test ($\mathcal{D}_T$) data do not follow the same distribution \cite{Redko2020_DASurvey}. Formally, $P_S(\mathbf{S}, \mathbf{X}, Y) \neq P_T(\mathbf{S}, \mathbf{X}, Y)$, where $P$ denotes the probability distribution over $\mathbf{S}\times\mathbf{X}\times Y$ and its subscript the corresponding domain. Given our notation {\bettina %$\leftarrow$ 
I would omit this starting clause}, it follows that $\mathcal{D}_S \sim P_S(\mathbf{S}, \mathbf{X}, Y)$ and $\mathcal{D}_T \sim P_T(\mathbf{S}, \mathbf{X}, Y)$. Changes between the distributions are referred to as \textit{distribution shifts}. There are three types of distributions shifts \cite{Quinonero2009,DBLP:journals/pr/Moreno-TorresRACH12}. \textit{Covariate shift}: only the distribution of the attributes changes, $P_S(Y | \mathbf{S}, \mathbf{X}) = P_T(Y | \mathbf{S}, \mathbf{X})$ but $P_S(\mathbf{S}, \mathbf{X}) \neq P_T(\mathbf{S}, \mathbf{X})$. \textit{Prior probability shift}: only the distribution of the label changes, $P_S(\mathbf{S}, \mathbf{X}|Y) = P_T(\mathbf{S}, \mathbf{X}|Y)$ but $P_S(Y) \neq P_T(Y)$. And \textit{dataset shift}: when none of the two previous cases apply but the joint distributions differ, $P_S(Y, \mathbf{S}, \mathbf{X}) \neq P_T(Y, \mathbf{S}, \mathbf{X})$.
% \begin{itemize}
%     \item \textit{Covariate shift}: only the distribution of the attributes changes, $P_S(Y | \mathbf{S}, \mathbf{X}) = P_T(Y | \mathbf{S}, \mathbf{X})$ but $P_S(\mathbf{S}, \mathbf{X}) \neq P_T(\mathbf{S}, \mathbf{X})$;
%     \item \textit{Prior probability shift}: only the distribution of the label changes, $P_S(\mathbf{S}, \mathbf{X}|Y) = P_T(\mathbf{S}, \mathbf{X}|Y)$ but $P_S(Y) \neq P_T(Y)$; and
%     \item \textit{Dataset shift}: when none of the two previous cases apply but the joint distributions differ, $P_S(Y, \mathbf{S}, \mathbf{X}) \neq P_T(Y, \mathbf{S}, \mathbf{X})$.
% \end{itemize}

We focus on the covariate shift type \cite{DBLP:conf/icml/ZhangSMW13}. In particular, we consider its \textit{unsupervised case} in which we only have access to the attribute space of $D_T$, meaning $Y \notin \mathcal{D}_T$. For simplicity, we also focus on the single source problem; see \cite{DBLP:conf/aaai/ZhangGS15} for a multi-source setting. Our focus here is due to the overall selection bias process we are considering, in which the class $Y$ is only available for the source domain instances as these are the instances previously selected by $\zeta$ and, consequently, already exposed to the data generating model behind $Y$. For example, we consider the case of a supermarket looking to target new clients ($D_T$) using what it knows about its current clients ($D_S$). In this case, the supermarket has access to the purchasing habits of its clients ($Y$) because they have purchased at the supermarket before ($\zeta=1$); this is not the same for the potential new clients. If both domains followed the same distribution, then we could ignore our lack of information on $D_T$ and generalize from $D_S$. Under covariate shift, however, this approach would lead to a biased model when used on the target domain. The best we can do is access the attribute space of $D_T$, which is generated separately from $Y$, and account for the potential distribution shift between $P_S(\mathbf{S}, \mathbf{X})$ and $P_T(\mathbf{S}, \mathbf{X})$ while assuming $P_S(Y|\mathbf{S}, \mathbf{X}) = P_T(Y|\mathbf{S}, \mathbf{X})$. \ja{ Add a causal graph: Appendix.}

{\bettina But given this construction of the problem, you'll then have to evaluate (a) your adaptation strategy but also (b) your assumption that this is really a covariate shift setting and not a dataset shift one?!}

\subsection{Entropy for Decision Tree Learning}
\label{sec:sec:ProblemSetting.DecisionTreeLearning}

Decision trees \cite{Hastie2009_ElementsSL} are intuitive, interpretable, and popular classification models. Top-down decision tree induction
algorithms grow a decision tree from the root to the leaves. At each node, either the growth stops 
%(if some stopping criterion is met, such as large purity or low number of cases) 
or child sub-trees are created based on a split criterion. The splitting attribute $X$ (and its corresponding threshold value $x$) is chosen by maximizing the split criteria. This step is done recursively given the \textit{current path} $\varphi$, where $\varphi$ is the conjunction of split conditions from the root of the decision tree up to the current node. In other words, $\varphi$ determines the partition of the data being explored at the current node.

We focus on the information gain split criterion. It is, along with Gini, one of the standard split criteria used. It is also based on information theory via entropy \cite{Cover1999ElementsIT}, which links a random variable's distribution to its information content. Such link allows us to address the domain adaptation problem of selection bias under the decision tree setting. \textit{Entropy} ($H$) measures the information contained within a random variable based on the uncertainty of its events. The standard definition used is \textit{Shannon's entropy} \cite{DBLP:conf/icaisc/MaszczykD08} where we define $H$ for a random variable $X$ as:
%
\begin{equation}
\label{eq:ShannonEntropy}
    H(X) = \sum_{x \in X} - P(X=x) \log_2(P(X=x))
\end{equation}
%
where $-\log_2(P(x))=I(x)$ represents the \textit{information} ($I$) of $X=x$. Therefore, entropy is the expected information of a random variable. The information of event $x$ is inversely proportional to its probability $P(x)$. The more certain the event $x$ is, reflected by a higher $P(x)$, the lower its information as $I(x)$ (along with $H(x)$) approaches 0. The general idea behind this is that there is little (new) information to be learned from an event that is certain to occur. 
We picture it as \textit{low entropy implies no surprises}. We will come back to this in the next section.

\ja{ Based on talk 20/12/2022: In later sections, we need to specify that \eqref{eq:ShannonEntropy}'s $P(X=x)$ weights is also from the target domain. Meaning that when we adapt the $IG$, we also have to enter the conditional entropy due to how the decision tree is learned and our assumption of covariate shift (which implies that $P_S(Y|\mathbf{X}) = P_T(Y|\mathbf{X})$).}

{\bettina From here on, I get a bit confused because of the notation. P(x) seems to be an unconditional probability of x (in the whole population), but the one you need is the probability at the end point of the current path, right? I.e., shouldn't P(x) be conditioned on the path? You say that somewhere further down, but I still find this notation confusing.}


For learning the decision tree, we define \textit{information gain} ($IG$) using \eqref{eq:ShannonEntropy} for the current path $\varphi$ and the attribute under splitting consideration $X$ as:
%
\begin{align}
\label{eq:BasicIG}
    IG(\varphi, X) 
    &= H(\varphi) - H(\varphi | X) \nonumber \\
    &= H(\varphi) - \sum_{x \in X} P(x) H(\varphi|x)
\end{align}
%
where the first term denotes the current (parent) node entropy and the second term the potential (child) node entropy by incorporating $X$ into $\varphi$ -- hence, the conditional entropy term. $IG$ is defined as the reduction of entropy of a given split.\footnote{This is because we can rewrite \eqref{eq:BasicIG} as
%\small
\begin{equation*}
    IG = -\sum_{i \in \varphi} P(\varphi_i)\log_2(P(\varphi_i)) + \sum_{x \in X} P(x) \sum_{i \in \varphi} P(\varphi_i|x) \log_2(\varphi_i|x)
\end{equation*}
meaning that when we minimize $IG$ we are actually maximizing the child node's entropy relative to the parent node.}
Under $IG$, we grow the decision tree under $X$ and its threshold value $x$ if it provides more information than $\varphi$ as it currently stands. This procedure is done for all attributes in $\mathbf{X}$ (and, also, in $\mathbf{S}$ under our setting) available for splitting at $\varphi$, where we choose the best one. 

\ja{ With this last comment in mind, we should maybe rewrite \eqref{eq:BasicIG} in terms of probabilities (as in the footnote) and later on in the decision-tree learning part, talk in terms of right and left hand side splits and source/target domain information gains.}

Notice that $IG$ is a random variable as both entropy terms in \eqref{eq:BasicIG} are random variables too. In terms of domain adaptation, standard decision tree learning implies that $IG(X, \varphi) \sim D_S$.
{\bettina Does the $\sim$ here mean the same as above?}
With that in mind, we highlight the second term's \textit{probability weight} $P(x)$ from the second line of \eqref{eq:BasicIG}. \textit{It denotes the probability of the conditional entropy for the new current path under consideration}. 
{\bettina probability of entropy?}
$H(\varphi|x)$ represents the information gained by appending $X$ with threshold value $x$ 
{\bettina threshold value? isn't it equal to $x$?}
to the existing conjunction of split conditions contained in $\varphi$, and $P(x)$ represents how probable this is to occur.\footnote{This weight comes from the fact that we are taking the expectation of a function of a random variable. See Appendix~\ref{appendix:WeightOrigin} for details.} For the same $H(\varphi | x)$, $H(\varphi | X)$ can increase (or decrease) depending on the weight $P(x)$. 
{\bettina unclear sentence: for the same A, A can be not the same depending on some B?}
In standard decision tree learning, this fact is useless as $P(x)$ cannot change for the same $x$ under the same $\varphi$ when we are using the same data $\mathcal{D}_S$. $P(x)$ is deterministic under these condition. Given our scenario of (unsupervised) covariate shift, however, this weight becomes 
interesting
%BB of interest 
granted we have some access to the data $\mathcal{D}_T$.  
{\bettina granted that = even assuming that -- are you sure this is what you mean? }

We propose modifying $P(x)$ in \eqref{eq:BasicIG} as a domain-adaptive weight. We can then incorporate information from $D_T$ when learning the decision tree, reducing the potential selection bias. As the tree grows, it is $P(x)$ that weights the contribution of the proposed splits and, consequently, influences the the structure of the final tree. Given that $P(x) \sim D_S$ and $P_S(\mathbf{X}) \neq P_T(\mathbf{X})$, we want the contributions from the proposed splits to be weighted with respect to $D_T$. Therefore, we want to modify $P(x)$ such that $P(x) \sim D_T$ (based on the target domain only) or, at least, $P(x) \sim D_S \cap D_T$ (based on a mixture of both domains) depending on the content of the data $\mathcal{D}_T$. That way, we grow a decision tree more representative of its intended population. %We introduce the domain-adaptive weight in the next section.

{\bettina What happened to the protected attributes S -- they seem to have disappeared?}

\subsection{Measures of Interest}
\label{sec:sec:ProblemSetting.Measures}

The goal is to obtain a decision tree classifier, based on the proposed modification to $IG$, that is both \textit{performant} and \textit{fair} on its intended population. The quality of the classifier's predictions, $\hat{Y}$, both in terms of performance and fairness, is measured relative to the 
ground truth,
%BB groundtruth, 
$Y$, of the instances in the test set (while the classifier itself is trained on the mutually exclusive training set). For classification models, this is implemented by using the elements of the confusion matrix \cite{Hastie2009_ElementsSL}: the number of true positives (TP), false positives (FP), true false negatives (FN), and true negatives (TN).\footnote{$TP \equiv \{ Y=1 \land \hat{Y}=1 \}$ and $FP \equiv \{ Y=0 \land \hat{Y}=1 \}$; the rest follow analogously.} In our case, how we measure performance and fairness will depend on our access to $\mathcal{D}_T \in D_T$, meaning on a case by case basis. 
{\bettina That sounds strange and potentially dangerous (hand-waving: we decide ad lib how to determine fairness). I believe you mean something else, but I don't know what.}
We will specify when needed during our implementation; here, we just present the measures of interest.

\textcolor{red}{For model performance}, we use \dots because \dots . Other possible performance metrics include: accuracy ($\frac{TP + TN}{TP + FP + FN + TN}$), precision ($\frac{TP}{TP + FP}$), recall or sensitivity ($\frac{TP}{TP + FN}$), specificity ($\frac{TN}{TN + FP}$), and F1 score, among others. 

For model fairness, we focus on\textit{ group-level metrics} focused around one of the $m$ sensitive attributes in $\mathbf{S}$ \cite{barocas-hardt-narayanan2019}. For illustrative purposes, consider a single discrete sensitive attribute $S$, such that $S=1$ denotes membership to the protected group and $S=0$ otherwise. If we are in the situation where $Y \notin \mathcal{D}_T$, we use \textit{demographic parity} (DP): $P(\hat{Y} | \mathbf{X}, S=1) = P(\hat{Y} | \mathbf{X}, S=1)$. 
{\bettina I think you need to correct this formula :-)}
The classifier is fair if $S$ does not condition the positive predicted outcome across the sub-populations of interest. Otherwise, if we have access to $Y \in \mathcal{D}_T$, we also use \textit{equal opportunity} (EO): $TPR_{S=1} = TPR_{S=0}$, where $TPR$ is the true positive rate ($\frac{TP}{TP+FN}$).
{\bettina would be easier to read if you used the same notation as for demographic parity.}
The classifier is fair if it has the same probability of predicting a positive outcome for outcomes that are actually positive across the sub-populations of interest.  

{\bettina Wouldn't that be "the classifier is perfectly fair if ..." - because in real life, of course the best you can do is approximate that?}

%
% EOS
%


==> previous_version/introduction_BB.tex <==
{\bettina I wrote this as a proposal for an intro. References are indicate in the cite environments; they still need to go into the bibtex of course. Please check whether you agree with them / whether you can provide something else.}

Invisibility can be unfair, and adequate visibility can be a prerequisite for fairness. This relationship has been observed since the early days of discrimination-aware and fairness-aware machine learning and data mining. A classic example is that of demographics such as female and darker-skinned people being underrepresented in computer-vision datasets – hence scarcely visible to the learning algorithm, with consequences such as high error rates in facial recognition and consequent denials of benefits (such as authentication) or imposition of harms (such as arrests) \cite{gender shades? Or something newer?}. The problem has been discussed as a selection bias, and sociological and psychological reasons for such selection biases have been identified \cite{Data Feminims book}. 

Selection bias implies that the training and test sets do not follow the same statistical distribution. Traditionally, this has been viewed as a bug in machine-learning setups, to be addressed by ``more representative data collection''. However, methods for transfer learning start from such differences as a feature. Transfer learning is becoming increasingly popular in practical applications due to the economic advantages of re-using existing model, but this poses the risk of imposing selection biases that lead to unfairness. We propose that transfer learning strategies should take such effects into account – and that they can profit from this awareness. 

We introduce {\em domain-adaptive decision trees} as a method for transfer learning to address these issue.  
We focus on decision trees given their popularity, interpretability relative to other ML models, and known statistical properties. We propose an in-processing step that augments the Information Gain (IG) split criterion with outside information corresponding to the target population we aim for. 
The approach works by adapting probabilities of child nodes to the target domain and in this sense by making parts of the feature space (such as certain demographics) more visible to the learning algorithm. We investigate the conditions in which this strategy can lead to increases in performance, in fairness, or in both.

We study two examples of settings in which transfer learning can yield benefits and produce unfairness. The first example uses the FolkTables dataset \cite{please supply}. The source and target domains are geographical regions that may have different demographic distributions. Here, bias and unfairness could surface in the well-studied forms of allocative harms (e.g. not being granted a loan) {\bettina NEEDS REF. – AND: I REALISE I NEED TO DISCUSS THIS ONCE MORE WITH YOU}. The second example uses a real-life retail dataset. The bias here is that marketing decisions made will be geared towards existing customers, rather than towards the current makeup of the local population. If those two groups are too different, stores may both fail to meet the needs of the local residents, possibly resulting into lower service or higher prices for some social groups, and lose opportunities to gain and retain customers amongst local residents.

The paper is organized as follows. TODO


